De Morgan Dual Nominal Quantifiers Modelling Private Names in Non-Commutative Logic

This paper explores the proof theory necessary for recommending an expressive but decidable first-order system, named MAV1, featuring a de Morgan dual pair of nominal quantifiers. These nominal quantifiers called `new' and `wen' are distinct from the self-dual Gabbay-Pitts and Miller-Tiu nominal quantifiers. The novelty of these nominal quantifiers is they are polarised in the sense that `new' distributes over positive operators while `wen' distributes over negative operators. This greater control of bookkeeping enables private names to be modelled in processes embedded as formulae in MAV1. The technical challenge is to establish a cut elimination result, from which essential properties including the transitivity of implication follow. Since the system is defined using the calculus of structures, a generalisation of the sequent calculus, novel techniques are employed. The proof relies on an intricately designed multiset-based measure of the size of a proof, which is used to guide a normalisation technique called splitting. The presence of equivariance, which swaps successive quantifiers, induces complex inter-dependencies between nominal quantifiers, additive conjunction and multiplicative operators in the proof of splitting. Every rule is justified by an example demonstrating why the rule is necessary for soundly embedding processes and ensuring that cut elimination holds.

==> LemmaBranching.tex <==
\proof{
The proof works by constructing two proofs such that the respective left and right formula of the with connective are removed.
To do so, we remove deductive rules that either involve the with connective concerned, or appear inside the branch to be removed. We provide only the case where the left branch is selected, the other case is symmetric. The function $\ell( . )$ over predicates with a distinguished \textit{bold with} operator $\boldsymbol\wwith$ is required. Where $\ell$ is defined such that $\ell( P \boldsymbol\wwith Q ) = P$, $\ell( P \odot Q ) = \ell(P) \odot \ell(Q)$, $\ell( \quantifier x P ) = \quantifier x \ell(P)$ and $\ell(\kappa) = \kappa$, where $\quantifier \in \left\{ \new, \wen, \forall, \exists \right\}$, $\odot \in \left\{ \ooplus, \wwith, \cpar, \cseq, \tensor \right\}$ and $\kappa \in \left\{ \cunit, \alpha, \co{\alpha} \right\}$.

The induction hypothesis is that if $\vdash T$, then we can construct a proof for $\vdash \ell(T)$.
The base case is when $\ell(T) = T$ (e.g.\ when $T = \cunit$), in which case we are done. The inductive cases are listed below.
\medskip

Consider when the bottommost rule of a proof
$
\context{ T \boldsymbol{\wwith} \contextb{U} } \longrightarrow \context{ T \boldsymbol{\wwith} \contextb{V} }
$
involving a bold \textit{with} such that $\vdash \context{ T \boldsymbol\wwith \contextb{V} }$.
Hence, by the induction hypothesis, $\vdash \ell\left( \context{ T  \boldsymbol\wwith \contextb{V} } \right)$ holds. Furthermore, $\ell\left( \context{ T  \boldsymbol{\wwith} \contextb{V} } \right) = \ell\left( \context{ T  \boldsymbol{\wwith} \contextb{U} } \right)$. Hence $\vdash \ell \left( \context{ T \boldsymbol{\wwith} \contextb{U} } \right)$ holds, as required.
\medskip

Consider when the bottommost rule of a proof
$
\context{ \left( T \boldsymbol\wwith U \right) \cpar V } \longrightarrow \context{ \left( T \cpar V \right) \boldsymbol\wwith \left( U \cpar V \right) }
$
 involving a bold \textit{with} such that
$\vdash \context{ \left( T \cpar V \right) \boldsymbol\wwith \left( U \cpar V \right) }$. 
Hence $\vdash \ell\left(\context{ \left( T \cpar V \right) \boldsymbol\wwith \left( U \cpar V \right) }\right)$ holds by the induction hypothesis.
Furthermore,  clearly
$\ell\left( \context{ \left( T \cpar V \right) \boldsymbol\wwith \left( U \cpar V \right) } \right) = \ell \left( \context{ \left( T \boldsymbol\wwith U \right) \cpar V } \right)$. Thereby $\vdash \ell\left( \context{ \left( T \boldsymbol\wwith U \right) \cpar V } \right)$ holds, as required.
\medskip

%%%%%% medial case %%%%%
Consider when the bottommost rule of a proof 
$
\context{
 \left( T \cseq U \right) \boldsymbol\wwith \left(V \cseq W\right)
}
\longrightarrow
\context{
 \left( T \boldsymbol\wwith V \right) \cseq \left( U \boldsymbol\wwith W \right)
}
$
involving a bold \textit{with} operator such that 
$
\vdash
\context{
 \left( T \boldsymbol\wwith V \right) \cseq \left( U \boldsymbol\wwith W \right)
}
$.
By the induction hypothesis, $
\vdash \ell\left(
 \context{
 \left( T \boldsymbol\wwith V \right) \cseq
 \left( U \boldsymbol\wwith W \right) }
\right)
$ holds. Furthermore, it is clear that
$
\ell\left(
 \context{
 \left( T \boldsymbol\wwith V \right) \cseq
 \left( U \boldsymbol\wwith W \right) }
\right)
=
\ell\left(
 \context{
 \left( T \cseq U \right) \boldsymbol\wwith
 \left( V \cseq W \right) }
\right)
$. Thereby $\vdash
\ell\left(
 \context{
 \left( T \cseq U \right) \boldsymbol\wwith
 \left( V \cseq W \right) }
\right)
$ holds, as required.
\medskip
%%%%%% end medial case %%%%%%%



%%%%%% wen case %%%%%
Consider when the bottommost rule of a proof 
$
\context{
 \wen x P \boldsymbol\wwith \wen x Q
}
\longrightarrow
\context{
 \wen x \left( P \boldsymbol\wwith Q \right)
}
$
involving a bold \textit{with} operator such that
$
\vdash
\context{
 \wen x \left( P \boldsymbol\wwith Q \right)
}
$. 
By the induction hypothesis, $
\vdash \ell\left(
 \context{
   \wen x \left( P \boldsymbol\wwith Q \right) 
}
\right)
$ holds. Furthermore, it is clear that
$
\ell\left(
 \context{
  \wen x P
}
\right)
=
\ell\left(
 \context{
    \wen x \left( P \boldsymbol\wwith Q \right)
}\right)
$. Thereby $\vdash
\ell\left(
 \context{
   \wen x \left( P \boldsymbol\wwith Q \right) 
}
\right)
$ holds, as required.
\medskip
%%%%%% end wen case %%%%%%%



%%%%%% wen case %%%%%
\ross{This case requires vacous wen lemma. Include in body of paper.}
Consider when the bottommost rule of a proof 
$
\context{
 P \boldsymbol\wwith \wen x Q
}
\longrightarrow
\context{
 \wen x \left( P \boldsymbol\wwith Q \right)
}
$
involving a bold \textit{with} operator, where $\nfv{x}{P}$.
Since $
\vdash
\context{
 \wen x \left( P \boldsymbol\wwith Q \right)
}
$,
by the induction hypothesis, $
\vdash \ell\left(
 \context{
   \wen x \left( P \boldsymbol\wwith Q \right) 
}
\right)
$ holds and also 
$
\ell\left(
 \context{
  \wen x \left( P \boldsymbol\wwith Q \right) 
}
\right)
=
\ell\left(
 \context{
   \wen x P
}\right)
$; 
hence $\vdash
\ell\left(
 \context{
   \wen x P
}
\right)
$ holds.
Now, by Lemma~\ref{lemma:vacuous-wen},
$\vdash
\ell\left(
 \context{
   P
}
\right)$ holds, since $\nfv{x}{P}$;
and 
$
\ell\left(
 \context{
   P
} \right)
=
\ell\left(
\context{
 P \boldsymbol\wwith \wen x Q
}\right)$;
thereby 
$
\vdash
\ell\left(
\context{
 P \boldsymbol\wwith \wen x Q
}\right)$
as required.
\medskip
%%%%%% end wen case %%%%%%%


%%%%%% new case %%%%%
Consider when the bottommost rule of a proof 
$
\context{
 \new x P \boldsymbol\wwith \new x Q
}
\longrightarrow
\context{
 \new x \left( P \boldsymbol\wwith Q \right)
}
$
involving a bold \textit{with} operator such that
$
\vdash
\context{
 \new x \left( P \boldsymbol\wwith Q \right)
}
$. 
By the induction hypothesis, $
\vdash \ell\left(
 \context{
   \new x \left( P \boldsymbol\wwith Q \right) 
}
\right)
$ holds. Furthermore, it is clear that
$
\ell\left(
 \context{
  \new x P
}
\right)
=
\ell\left(
 \context{
    \new x \left( P \boldsymbol\wwith Q \right)
}\right)
$. Thereby $\vdash
\ell\left(
 \context{
   \new x \left( P \boldsymbol\wwith Q \right) 
}
\right)
$ holds, as required.
\medskip
%%%%%% new case %%%%%%%



%%%%%% new case %%%%%
Consider when the bottommost rule of a proof 
$
\context{
 P \boldsymbol\wwith \new x Q
}
\longrightarrow
\context{
 \new x \left( P \boldsymbol\wwith Q \right)
}
$
involving a bold \textit{with} operator, where $\nfv{x}{P}$.
Since $
\vdash
\context{
 \new x \left( P \boldsymbol\wwith Q \right)
}
$,
by the induction hypothesis, $
\vdash \ell\left(
 \context{
   \new x \left( P \boldsymbol\wwith Q \right) 
}
\right)
$ holds and also 
$
\ell\left(
 \context{
  \new x \left( P \boldsymbol\wwith Q \right) 
}
\right)
=
\ell\left(
 \context{
   \new x P
}\right)
$; 
hence $\vdash
\ell\left(
 \context{
   \new x P
}
\right)
$ holds.
Now, by Lemma~\ref{lemma:vacuous-new},
$\vdash
\ell\left(
 \context{
   P
}
\right)$ holds, since $\nfv{x}{P}$;
and 
$
\ell\left(
 \context{
   P
} \right)
=
\ell\left(
\context{
 P \boldsymbol\wwith \new x Q
}\right)$;
thereby 
$
\vdash
\ell\left(
\context{
 P \boldsymbol\wwith \new x Q
}\right)$
as required.
\medskip
%%%%%% wen case %%%%%%%







Consider the case where $\context{ \cunit \boldsymbol\wwith \cunit } \longrightarrow \context{ \cunit }$, where $\vdash \context{ \cunit }$. By the induction hypothesis, $\vdash\ell \left( \vdash \context{ \cunit } \right)$ holds. Furthermore $\ell \left( \context{ \cunit \boldsymbol\wwith \cunit } \right) = \ell \left( \context{ \cunit } \right)$; hence $\vdash \ell \left( \context{ \cunit \boldsymbol\wwith \cunit } \right)$ as required.

In all other cases, $\context{ T } \longrightarrow \context{ U }$, by any rule, such that $\vdash \context{ T }$ and also $\ell \left( \context{T} \right) \not\equiv \ell \left( \context{U} \right)$.
By induction, $\vdash \ell \left( \context{ U } \right)$ holds. Therefore, by applying the same rule, we can obtain a proof of $\ell\left( U \right)$.
\medskip

All cases are exhausted, thereby if $\vdash T$ holds then $\vdash \ell(T)$ for any length of proof. Whence, by assuming that $\context{ T \boldsymbol\wwith U }$ holds, we can construct a proof of $\ell \left(\context{ T \boldsymbol\wwith U }\right) = \context{ T }$. A symmetric argument using a right projection on the bold \textit{with} operator constructs a proof of $\context{ U }$.
}



==> killing-medial-proof.tex <==
\begin{proof}
The proof is by induction on the structure of $\tcontext{}$.
The base case is immediate.

Assume that $\tcontext{}$ is a $n$-ary killing context and $P_i$ and $Q_i$ are such that $\nfv{x}{P_i}$ and either $P_i = \wen x. Q_i$ or $P_i = Q_i$,
for $1 \leq i \leq n$; and also for some $i$ such that $1 \leq i \leq n$, $P_i = \wen x. Q_i$.
By the induction hypothesis, $\tcontext{ P_1, P_2, \hdots P_n} \longrightarrow \wen x. \tcontext{ Q_1, Q_2, \hdots, Q_n }$.
Hence the following derivation can be constructed for $\new$.
\[
\new y. \tcontext{ P_1, P_2, \hdots P_n } \longrightarrow \new y. \wen x. \tcontext{ Q_1, Q_2, \hdots, Q_n }
\longrightarrow \wen x. \new y. \tcontext{ Q_1, Q_2, \hdots, Q_n }
\]
Similarly, the following derivation can be constructed for $\forall$.
\[
\forall y. \tcontext{ P_1, P_2, \hdots P_n } \longrightarrow \forall y. \wen x. \tcontext{ Q_1, Q_2, \hdots, Q_n }
\longrightarrow \wen x. \forall y. \tcontext{ Q_1, Q_2, \hdots, Q_n }
\]

Now assume that $\tcontextn{0}{}$ and $\tcontextn{1}{}$ are respectively $m$-ary and $n$-ary killing contexts and $P_i$ and $Q_i$ are such that $\nfv{x}{P_i}$ and either $P_i = \wen x. Q_i$ or $P_i = Q_i$,
for $1 \leq i \leq m+n$; and also for some $i$ such that $1 \leq i \leq m+n$, $P_i = \wen x. Q_i$.
Assume that, for some $j$ such that $1 \leq j \leq m$, $P_j = \wen x Q_j$. By induction, we have the following derivation.
$
\tcontextn{0}{ P_1, \hdots, P_m } \longrightarrow \wen x. \tcontextn{0}{ Q_1, \hdots, Q_m }
$.

Now assume also that there exists $k$ such that $m+1 \leq k \leq m+n$ and $P_k = \wen x. Q_k$.
In the first case, by induction, the following derivation holds.
$
\tcontextn{1}{ P_{m+1}, \hdots, P_{m+n} } \longrightarrow \wen x. \tcontextn{1}{ Q_{m+1}, \hdots, Q_{m+n} }
$.

In this case, the following derivation can be constructed.
\[
\begin{array}{rl}
\tcontextn{0}{ P_1, \hdots, P_m }
\wwith
\tcontextn{1}{ P_{m+1}, \hdots, P_{m+n} }
\longrightarrow&
\wen x. \tcontextn{0}{ Q_1, \hdots, Q_m }
\wwith
\wen x. \tcontextn{1}{ Q_{m+1}, \hdots, Q_{m+n} }
\\
\longrightarrow&
\mathopen{\wen x.} \left(\tcontextn{0}{ Q_1, \hdots, Q_m }
\wwith
\tcontextn{1}{ Q_{m+1}, \hdots, Q_{m+n} }\right)
\end{array}
\]
Otherwise $P_\ell = Q_\ell$, hence $\nfv{x}{Q_\ell}$, for all $\ell$ such that $m+1 \leq \ell \leq m+n$. Thereby $\nfv{x}{\tcontextn{1}{Q_1, \hdots, Q_n}}$ and hence the follow derivation holds.
\[
\begin{array}{rl}
\tcontextn{0}{ P_1, \hdots, P_m }
\wwith
\tcontextn{1}{ P_{m+1}, \hdots, P_{m+n} }
\longrightarrow&
\wen x. \tcontextn{0}{ Q_1, \hdots, Q_m }
\wwith
\tcontextn{1}{ Q_{m+1}, \hdots, Q_{m+n} }
\\
\longrightarrow&
\mathopen{\wen x.} \left(\tcontextn{0}{ Q_1, \hdots, Q_m }
\wwith
\tcontextn{1}{ Q_{m+1}, \hdots, Q_{m+n} }\right)
\end{array}
\]
The third case when $P_\ell = Q_\ell$ for all $\ell$ such that $1 \leq \ell \leq m$ is symmetric.
\end{proof}


==> multiset2.tex <==
%\paragraph{Termination Lemmas.}

%The following notable lemma, will be used to deal with a troublesome case concerning the interaction between associativity of seq and partial distributivity of the additives. For now, consider Lemma~\ref{lemma:main-case} as a substantial example of applying the above lemmas for multisets.
The following lemma is required for the principal case for \textit{seq}.
\begin{lemma}\label{lemma:main-case}
Assume that $T_0 \not\equiv \cunit$, $T_2 \not\equiv \cunit$ and, either $U \not\equiv \cunit$ or $V \not\equiv \cunit$, and the derivation
$
W \longrightarrow \tcontext{P_i \cseq Q_i \colon 1 \leq i \leq n}
$  hold.

There are two symmetric cases to consider. For the first case, also assume that the derivation 
$
V \cpar Q_i \longrightarrow \tcontextn{i}{R^i_j \cseq S^i_j \colon 1 \leq j \leq m_i}
$ holds for every $i$.
In this case, the following two strict multiset inequalities hold.
\[
%\begin{array}{l}
\size{
 \left(T_0 \cseq T_1\right) \cpar \left(\left( U \cpar P_i \right) \cseq \tcontextn{i}{R^i_j \colon 1 \leq j \leq m_i}\right)
}
\mstrict
\size{
 \left(T_0 \cseq T_1 \cseq T_2\right) \cpar \left( U \cseq V \right) \cpar W
}
%\end{array}
\]
\[
\size{ T_2 \cpar \tcontextn{i}{ S^i_j \colon 1 \leq j \leq m_i} }
\mstrict
\size{
 \left(T_0 \cseq T_1 \cseq T_2\right) \cpar \left( U \cseq V \right) \cpar W
}
\]
For the second case, symmetric to the above. Instead assume that the derivation 
$
U \cpar P_i \longrightarrow \tcontextn{i}{R^i_j \cseq S^i_j \colon 1 \leq j \leq m_i}
$ holds for every $i$.
In this second case, the following two strict multiset inequalities hold.
\[
%\begin{array}{l}
\size{
 \left(T_1 \cseq T_2\right) \cpar \left( \tcontextn{i}{S^i_j \colon 1 \leq j \leq m_i} \cseq \left( Q_i \cpar V \right) \right)
}
%\\\qquad\qquad\qquad\qquad\qquad
\mstrict
\size{
 \left(T_0 \cseq T_1 \cseq T_2\right) \cpar \left( U \cseq V \right) \cpar W
}
%\end{array}
\]
\[
\size{ T_0 \cpar \tcontextn{i}{ R^i_j \colon 1 \leq j \leq m_i} }
\mstrict
\size{
 \left(T_0 \cseq T_1 \cseq T_2\right) \cpar \left( U \cseq V \right) \cpar W
}
\]
\end{lemma}


==> proof_distribute.tex <==
\begin{proof}
The proofs follow by straightforward inductions over the structure of a killing context.

When the killing context is one hole only $P \cpar \ehole{Q} = \ehole{P \cpar Q}$ and $\ehole{\cunit} = \cunit$, as required.

Now assume that by the induction hypothesis the following hold for killing contexts $\tcontextn{1}{}$ and $\tcontextn{2}{}$, and also $\vdash \tcontextn{1}{\cunit, \hdots, \cunit}$ and $\vdash \tcontextn{2}{\cunit, \hdots, \cunit}$.
\[
\begin{array}{rl}
 P \cpar \tcontextn{1}{Q_1, \hdots, Q_m} &\longrightarrow \tcontextn{1}{P \cpar Q_1, \hdots, P \cpar Q_m}
 \\
 P \cpar \tcontextn{2}{Q_{m+1}, \hdots, Q_{m+n}} &\longrightarrow \tcontextn{2}{P \cpar Q_{m+1}, \hdots, P \cpar Q_{m+n}}
\end{array}
\]
Hence, by distributivity the following derivation can be constructed.
\[
\begin{array}{l}
P \cpar \left( \tcontextn{1}{Q_1, \hdots, Q_m} \wwith \tcontextn{2}{Q_{m+1}, \hdots, Q_{m+n}} \right)
\\\qquad
 \begin{array}{l}
 \longrightarrow P \cpar \tcontextn{1}{Q_1, \hdots, Q_m} \wwith P \cpar \tcontextn{2}{Q_{m+1}, \hdots, Q_{m+n}}
 \\
 \longrightarrow \tcontextn{1}{P \cpar Q_1, \hdots, P \cpar Q_m} \wwith \tcontextn{2}{P \cpar Q_{m+1}, \hdots, P \cpar Q_{m+n}}
 \end{array}
\end{array}
\]
Furthermore, $\tcontextn{1}{\cunit, \hdots, \cunit} \wwith \tcontextn{2}{\cunit, \hdots, \cunit} \longrightarrow \cunit \wwith \cunit \longrightarrow \cunit$ holds.

As the induction hypothesis, assume $P \cpar \tcontext{ Q_1, \hdots, Q_n } \longrightarrow \tcontext{ P \cpar Q_1, \hdots, P \cpar Q_n }$ and also that $\vdash \tcontext{ \cunit, \hdots, \cunit }$ . Hence, given $\nfv{x}{P}$, the following derivation holds.
\[
P \cpar \new x \tcontext{ Q_1, \hdots, Q_n } \longrightarrow \new x \left( P \cpar \tcontext{ Q_1, \hdots, Q_n }\right) \longrightarrow \new x \tcontext{ P \cpar Q_1, \hdots, P \cpar Q_n }
\]
Furthermore, $\new x \tcontext{ \cunit, \hdots, \cunit} \longrightarrow \new x \cunit \longrightarrow \cunit$.

A similar argument holds for a killing context of the form $\forall x \tcontext{}$.
\end{proof}


==> properties.tex <==

%Most of the following properties, required in proofs, are standard for multisets. The properties concerning multisets of multisets of natural numbers are treated more carefully.
\begin{lemma}\label{lemma:multisets}
Multiset orders, $\leq$ and $\mleq$ are precongruences.
Furthermore, the following properties hold for multisets of natural numbers $K$, $M$ and $N$ and multisets of multisets of natural numbers $\mathcal{K}$, $\mathcal{M}$ and $\mathcal{N}$.
\begin{gather*}
M + N = N + M
\qquad
(K + M) + N = K + (M + N)
\qquad
K + (M \cup N) = (K + M) \cup (K + N)
\\[6pt]
M \cup N = N \cup M
\qquad
(K \cup M) \cup N = K \cup (M \cup N)
\qquad
M + \left\{ 0 \right\} = M
\qquad
M < M \cup N
\\[6pt]
K + \mmax{ M, N } = \mmax{ K + M, K + N }
\qquad
\mmax{M, \mmax{N,K}} = \mmax{\mmax{M, N},K}
\\[6pt]
\mmax{M, \left\{0\right\}} = M
\qquad
\mmax{M, N}=\mmax{N,M}
%\qquad\mmax{ M \cup N, K } = \mmax{ M, K } \cup \mmax{ N, K }
\\[6pt]
\mbox{if } 
\left\{\left\{0\right\}\right\} \mstrict \mathcal{M}
\mbox{ and }
\left\{\left\{0\right\}\right\} \mstrict \mathcal{N}
\mbox{ then }
\mathcal{M} \cup \mathcal{N} \mstrict \mathcal{M} \mplus \mathcal{N}
\qquad
\mathcal{K} \mcup (\mathcal{M} \cup \mathcal{N}) =
\left(\mathcal{K} \mcup \mathcal{M}\right) \cup \left(\mathcal{K} \mcup \mathcal{N}\right)
\\[6pt]
\mathcal{K} \mplus (\mathcal{M} \mcup \mathcal{N}) =
\left(\mathcal{K} \mplus \mathcal{M}\right) \mcup \left(\mathcal{K} \mplus \mathcal{N}\right)
\qquad
\mathcal{K} \mplus (\mathcal{M} \cup \mathcal{N}) =
\left(\mathcal{K} \mplus \mathcal{M}\right) \cup \left(\mathcal{K} \mplus \mathcal{N}\right)
\end{gather*}
\end{lemma}
\begin{comment}
\proof{
Most properties are standard for multisets. We provide only proofs for the final four properties, which involve interactions between the two distinct multiset orderings.
\medskip

Firstly, assume that $\left\{\left\{0\right\}\right\} \mstrict \mathcal{M}$ and $\left\{\left\{0\right\}\right\} \mstrict \mathcal{N}$. Hence either $\left\{\left\{ 1 \right\}\right\} \mleq \mathcal{M}$ or $\left\{\left\{ 0, 0 \right\}\right\} \mleq \mathcal{M}$
and also either $\left\{\left\{1\right\}\right\} \mleq \mathcal{N}$ or $\left\{\left\{0, 0\right\}\right\} \mleq \mathcal{N}$. For any $M \in \mathcal{M}$ and $N \in \mathcal{N}$, we have that
\[
M \in \mathcal{M} \cup \mathcal{N}
\mbox{ and }
N \in \mathcal{M} \cup \mathcal{N}
\]
and also
\[
M + N \in \mathcal{M} \mplus \mathcal{N}
\]
Now, there are four cases to consider. If $\left\{ 0, 0 \right\} \leq M$ then $N < N \cup N = \left\{ 0, 0 \right\} + N \leq M + N$; and similarly if $\left\{ 0, 0\right\} \leq N$ then $M < M + N$. If $\left\{ 1 \right\} \leq M$ then $N < \left\{ 1 \right\} + N \leq M + N$; and similarly if $\left\{ 1 \right\} \leq N$ then $M < M + N$. In all cases $M < M+N$ and $N < M+N$. Hence $\mathcal{M} \cup \mathcal{N} \mstrict \mathcal{M} \mplus \mathcal{N}$.
\medskip

Secondly, consider every $M \in \mathcal{M}$, $N \in \mathcal{N}$, $K \in \mathcal{K}$, in which case the following hold.
\[
M \cup K \in
\left(\mathcal{M} \mcup \mathcal{K}\right) \cup \left(\mathcal{N} \mcup \mathcal{K}\right)
\mbox{ and }
N \cup K \in
\left(\mathcal{M} \mcup \mathcal{K}\right) \cup \left(\mathcal{N} \mcup \mathcal{K}\right)
\]
and also
\[
M \cup K \in
\left(\mathcal{M} \cup \mathcal{N}\right) \mcup \mathcal{K}
\mbox{ and }
N \cup K \in
\left(\mathcal{M} \cup \mathcal{N}\right) \mcup \mathcal{K}
\]
Hence $
\left(\mathcal{M} \mcup \mathcal{K}\right) \cup \left(\mathcal{N} \mcup \mathcal{K}\right)
=
\left(\mathcal{M} \cup \mathcal{N}\right) \mcup \mathcal{K}
$.
\medskip

Thirdly, consider distributivity of $\mplus$ over $\mcup$. In this case the following reasoning holds, as required.
\[
\begin{array}{rl}
\left(\mathcal{M} \mplus \mathcal{K}\right) \mcup \left(\mathcal{N} \mplus \mathcal{K}\right)
=&
\left\{ (M + K) \cup (N + K) \colon M \in \mathcal{M}, N \in \mathcal{N}, K \in \mathcal{K} \right\}
\\
=&
\left\{ (M \cup N) + K \colon M \in \mathcal{M}, N \in \mathcal{N}, K \in \mathcal{K} \right\}
\\
=&
\left(\mathcal{M} \mcup \mathcal{N}\right) \mplus \mathcal{K}
\end{array}
\]
\medskip

Fourthly, consider when $M \in \mathcal{M}$, $N \in \mathcal{N}$ and $K \in \mathcal{K}$. In this case the following holds
\[
 M + K \in \mathcal{K} \mplus \left(\mathcal{M} \cup \mathcal{N}\right)
\mbox{ and }
 N + K \in \mathcal{K} \mplus \left(\mathcal{M} \cup \mathcal{N}\right)
\]
and also
\[
 M + K \in \left(\mathcal{K} \mplus \mathcal{M}\right) \cup \left(\mathcal{K} \mplus \mathcal{N}\right)
\mbox{ and }
 N + K \in \left(\mathcal{K} \mplus \mathcal{M}\right) \cup \left(\mathcal{K} \mplus \mathcal{N}\right)
\]
Therefore $\mathcal{K} \mplus \left(\mathcal{M} \cup \mathcal{N}\right) = \left(\mathcal{K} \mplus \mathcal{M}\right) \cup \left(\mathcal{K} \mplus \mathcal{N}\right)$.
}
\end{comment}


%The key property of multisets is the distributivity of $+$ over $\cup$, from which we can establish $\size{\left(P \wwith Q\right) \cpar R} = \size{\left(P \cpar R\right) \wwith \left(Q \cpar R\right)}$. Thus, although the abstract syntax tree grows when the \textit{external} rule is applied, the multiset defined size of the predicate remains bounded by the size of the conclusion.

The following lemmas formalise the property of rewrite rules that rewriting reduces the size of the predicate, where Lemma~\ref{lemma:strict-times} and Lemma~\ref{lemma:strict-seq} emphasise the strict multiset inequality in these cases.
\begin{lemma}\label{lemma:strict-times}
Assuming that $P \not\equiv \cunit$ and $R \not\equiv \cunit$, the following strict multiset inequality holds.
\[
\occ{ P \tensor \left(Q \cpar R\right) }
\mstrict
\occ{ \left(P \tensor Q\right) \cpar R }
\]
\end{lemma}
\begin{comment}
\begin{proof}
If $Q \not\equiv \cunit$, then, since $R \not\equiv \cunit$ we have $\left\{\left\{ 0 \right\}\right\} \mstrict \occ{R}$ and hence $\occ{P} = \occ{P} \mplus \left\{\left\{ 0 \right\}\right\} \mstrict \occ{P} \mplus \occ{R}$; and therefore the following holds by Lemma~\ref{lemma:multisets}.
\[
\begin{array}{rl}
\occ{P \tensor \left(Q \cpar R\right)}
=& \occ{P} \cup \left( \occ{Q} \mplus \occ{R} \right)
\\
\mstrict& \left(\occ{P} \mplus \occ{R}\right) \cup \left( \occ{Q} \mplus \occ{R} \right)
\\
=& \left(\occ{P} \cup \occ{Q}\right) \mplus \occ{R}
= \occ{\left(P \tensor Q\right) \cpar R}
\end{array}
\]
If $Q \equiv \cunit$ then, since $\left\{\left\{0\right\}\right\} \mstrict \occ{P}$ and $\left\{\left\{0\right\}\right\} \mstrict \occ{R}$, the following holds by Lemma~\ref{lemma:multisets} and Lemma~\ref{lemma:multiset-congruence}.
\[
\occ{P \tensor \left( \cunit \cpar R\right)}
= \occ{P} \cup \occ{R}
\mstrict \occ{P} \mplus \occ{R}
= \occ{\left(P \tensor \cunit\right) \cpar R}
\]
\end{proof}
\end{comment}

\begin{lemma}\label{lemma:strict-seq}
Assuming that $Q \not\equiv \cunit$ and $R \not\equiv \cunit$ the following strict multiset inequality holds.
\[
\occ{\left(P \cpar R\right) \cseq \left(Q \cpar S\right)}
\mstrict
\occ{\left(P \cseq Q\right) \cpar \left(R \cseq S\right)}
\]
\end{lemma}
\begin{comment}
\begin{proof}
If $Q \not\equiv \cunit$ and $R \not\equiv \cunit$, then the following holds by Lemma~\ref{lemma:multisets}.
\[
\begin{array}{rl}
\occ{\left(P \cpar R\right) \cseq \left(Q \cpar S\right)}
=&\left( \occ{P} \mplus \occ{R} \right) \cup \left( \occ{Q} \mplus \occ{S} \right)
\\
\mstrict&\left( \occ{P} \mplus \occ{R} \right) \cup \left( \occ{Q} \mplus \occ{S} \right) \cup \left( \occ{P} \mplus \occ{S} \right) \cup \left( \occ{Q} \mplus \occ{R} \right)
\\
=&\left( \occ{P} \cup \occ{Q} \right) \mplus \left( \occ{R} \cup \occ{S} \right)
= \occ{\left(P \cseq Q\right) \mplus \left(R \cpar S\right)}
\end{array}
\]
If $Q \equiv \cunit$ and $R \not\equiv \cunit$, then, since $\left\{\left\{0\right\}\right\} \mstrict \occ{R}$, and hence $\occ{S} = \occ{S} \mplus \left\{\left\{0\right\}\right\} \mstrict \occ{S} \mplus \occ{R}$, therefore by Lemma~\ref{lemma:multisets} and Lemma~\ref{lemma:multiset-congruence} the following strict inequality holds.
\[
\begin{array}{rl}
\occ{\left(P \cpar R\right) \cseq \left(\cunit \cpar S\right)}
=&\left( \occ{P} \mplus \occ{R} \right) \cup \occ{S}
\\
\mstrict&\left( \occ{P} \mplus \occ{R} \right) \cup \left(\occ{S} \mplus \occ{R}\right)
\\
\mleq& \occ{P} \mplus \left( \occ{R} \cup \occ{S} \right)
=
\occ{\left(P \cseq \cunit \right) \mplus \left(R \cpar S\right)}
\end{array}
\]
A symmetric argument holds when $Q \not\equiv \cunit$ and $R \equiv \cunit$.

If $Q \equiv \cunit$ and $R \equiv \cunit$, then $\left\{\left\{0\right\}\right\} \mstrict \occ{P}$ and $\left\{\left\{0\right\}\right\} \mstrict \occ{S}$; hence the following strict inequality holds  by Lemma~\ref{lemma:multisets} and Lemma~\ref{lemma:multiset-congruence}.
\[
\begin{array}{rl}
\occ{\left(P \cpar \cunit\right) \cseq \left(\cunit \cpar S\right)}
= \occ{P} \cup \occ{S}
\mstrict \occ{P} \mplus \occ{S}
= \occ{\left(P \cseq \cunit \right) \cpar \left(\cunit \cseq S\right)}
\end{array}
\]
\end{proof}
\end{comment}


==> semantics.tex <==
\subsection{The Multiplicative Operators: Parallelism, sequentiality and interaction in \textsf{BV}}

The three multiplicative binary operators ``parallel'', ``synchronise'', and ``sequence'' form the sub-system \textsf{BV}~\cite{Guglielmi2007}. %, that \textsf{PV} conservatively extends.
Atoms, co-atoms and the multiplicatives can be provided with a processes calculus intuition. There is also the unit $\cunit$, which fulfils a number of roles. Unit is the left and right identity for all multiplicatives, as captured by the structural congruence. It will also fulfil the special role of representing `successful termination' and `classical true', which become clearer as this text progresses. 
%
The channel co-atom $\co{a(\textit{t})}$ (abbreviated $\co{a}(\textit{t})$) is similar to an output of constant $\textit{t}$ on channel $a$; while $a(\textit{t})$ represents an input of the same value $\textit{t}$ on channel $a$ of value $\textit{t}$. (Wait for quantifiers to understand input binders.)

Parallel composition or simply \textit{par}, allows atoms in processes composed in parallel to interact with each other. The ability for atoms to interact over parallel composition is represented by the two \textit{interaction} rules in Figure~\ref{figure:rewrite}. 
%
Sequential composition or simply \textit{seq}, indicates that all atoms on the left of the operator are ordered before all atoms on the right of the operator. If atoms represent events, then seq indicates that events on the left ``happen before'' events on the right~\cite{Lamport1979}. The seq rule, arising in the algebra of pomsets~\cite{Gischer1988}, decides a point in a protocol, where additional sequentiality is required. For example, the following derivation, familiar from interacting process calculi~\cite{Milner1989}, decides that the interaction of an atom and co-atom will ``happen before'' events represented by predicates $P$ and $Q$.
\[
\left(\co{a}(b) \cseq P\right) \cpar \left(a(b) \cseq Q\right)
\longrightarrow
\left(\co{a}(b) \cpar a(b)\right) \cseq \left(P \cpar Q\right)
\longrightarrow
P \cpar Q
\]
Note that interactions in the middle of processes are permitted such as the following.
\[
\begin{array}{rl}
\left(P \cseq \co{a}(b) \cseq Q\right) \cpar \left(R \cseq a(b) \cseq S\right)
%\longrightarrow& \left(P \cpar R\right) \cseq \left(\co{a}(b) \cpar a(b)\right) \cseq \left(Q \cpar S\right)\\
\longrightarrow&
\left(P \cpar R\right) \cseq \left(Q \cpar S\right)
\end{array}
\]
This is completely acceptable for static analysis where later parts of the protocol may be analysed first. The rewrite $\longrightarrow$ does not represent the causal order of events, instead causal dependencies are represented by sequential composition, as in a \textit{behavioural} model of concurrency~\cite{Sassone1996}.

Synchronise or simply ``sync'', also represents a stricter form of parallel composition or separation, where neither communication nor interleaving are permitted. That is, if an atom and co-atom are separated by a sync, then they may never interact. Also, atoms in one process may never be sequentially ordered with respect to atoms in another process. The effect is to model synchronisation in distributed systems, where two separate processes must execute their entirety within the same time frame. The switch rule, indicates the interplay between par and sync, by refining where interactions may or may not occur. 

As an example of sync, consider the following derivation.
\[
\begin{array}{l}
\co{a}(\textit{OK}) \cpar \left(\co{b}(\textit{OK}) \cseq c(\textit{t})\right)
\cpar
\left(a(\textit{OK}) \tensor b(\textit{OK})\right) \cseq \co{c}(\textit{t})
\\~~~~~~
\begin{array}{l}
\longrightarrow
\left(\co{a}(\textit{OK}) \cpar \co{b}(\textit{OK})\right) \cseq c(\textit{t})
\cpar
\left(a(\textit{OK}) \tensor b(\textit{OK})\right) \cseq \co{c}(\textit{t})
\\
\longrightarrow
\left(\co{a}(\textit{OK}) \cpar \co{b}(\textit{OK})
\cpar
\left(a(\textit{OK}) \tensor b(\textit{OK})\right)\right)
\cseq
\left( c(\textit{t}) \cpar \co{c}(\textit{t})\right)
\\
\longrightarrow
\left(
\co{b}(\textit{OK})
\cpar
\left(
\left(\co{a}(\textit{OK}) \cpar a(\textit{OK})\right) \tensor b(\textit{OK})
\right)
\right)
\cseq
\left( c(\textit{t}) \cpar \co{c}(\textit{t})\right)
\\
%\longrightarrow
%\left(
% \co{b}\,\textit{OK}
%\cpar b\,\textit{OK} \right)
%\cseq
%\left( c\,\textit{t} \cpar \co{c}\textit{t}\right)
%\\
\longrightarrow
\left(
\left(\co{a}(\textit{OK}) \cpar a(\textit{OK})\right) \tensor \left( \co{b}(\textit{OK})
\cpar b(\textit{OK}) \right)
\right)
\cseq
\left( c(\textit{t}) \cpar \co{c}(\textit{t})\right)
\\
\longrightarrow
\left( c(\textit{t}) \cpar \co{c}(\textit{t})\right)
\\
\longrightarrow
\cunit
\end{array}
\end{array}
\]
In the above, the inputs on channels $a$ and $b$ must both be completed atomically. Sync can be seen intuitively as a generalisation of $\tensor$ in synchronous process calculi such as SCCS~\cite{Milner1989}, where instead of all synchronous process performing an event in lockstep, several events may occur within the same time frame.

%Even if synchronisation is not regularly necessary for modelling protocols, the operator arises as the dual operator to par~\cite{Guglielmi2007}, resulting in a calculus with desirable proof theoretic properties explored in the second half of this paper.

\paragraph{An example of remote application protocol.}
%from Google file system.}
We are ready to express the first substantial example protocol.
In remote desktop applications, the interaction with the interface is often designed for a local desktop environment, hence latency can be high as the application waits for many messages to be sent over a wide-area network.

Consider the following data access protocol, that requests user details after discovering that the access-control policy required authentication. The first line represents the client front end and the second line the server back end.
\[
\begin{array}{rl}
&
\co{\textit{get\_file}} \cseq \textit{who} \cseq \co{\textit{here\_name}}
\cseq \textit{here\_file}
\\
\cpar
&
\textit{get\_file} \cseq \co{\textit{who}} \cseq \textit{here\_name} \cseq \co{\textit{here\_file}}
\end{array}
\]
The above protocol terminates after four messages exchanged over WAN. A mediator or \textit{branch repeater}~\cite{Zhang2012}
%\bogdan{the bibitem was missing so i added one; hope is the correct one}
can simulate several steps of the protocol at each endpoint thereby reducing the number of messages exchanged over WAN to two (\textit{rx} and \textit{tx} in the example below).
%
The following two lines describe the client and server sides of the branch repeater respectively.
\[
\begin{array}{rl}
&
\left(
 \left(
  \textit{get\_file} \cseq \co{\textit{who}} \cseq \textit{here\_name} \cseq \co{\textit{here\_file}}
 \right)
 \tensor
 \left(
  \co{\textit{tx}}
  \cseq
  \textit{rx}
 \right)
\right)
\\
\cpar
&
\left(
 \left(
  \textit{tx}
  \cseq
  \co{\textit{rx}}
 \right)
 \tensor
 \left(
  \co{\textit{get\_file}} \cseq \textit{who} \cseq \co{\textit{here\_name}} \cseq \textit{here\_file}
 \right)
\right)
\end{array}
\]
The original predicates describing the protocol and the predicate describing the branch repeater above, when composed in parallel, have a derivation that ends with the unit. Thereby the optimised protocol still works.
%A finer analysis is possible when the messages exchanged are made explicit. by using further features of the calculus.
See~\cite{Trubitsin2015} for related examples.


\begin{comment}
Consider a example of a simple client driven Two Phase Commit protocol. The client aims to perform an atomic transaction across two machines, known as the leader and participant. The participant....

!!! GFS example for diversity.

Assume there is one leader and one participants that must synchronise with the leader. Both participants make a prepare event observable (by sending a message) before receiving a commit message. We model the global protocol using the following formula.
\[
\begin{array}{c}
\left(
 \left(\textit{prepare} \tensor \textit{prepare}\right)
 \cseq
 \left( \co{\textit{commit}} \tensor \co{\textit{commit}} \right)
\right)
\cpar
\\
\left(
 \co{\textit{prepare}} \cseq \textit{commit}
\right)
\cpar
\\
\left(
 \co{\textit{prepare}} \cseq \textit{commit}
\right)
\end{array}
\]
The first line represents the leader, which coordinates the transaction. The second and third lines represent the protocol of the each of the participant. All three lines together represent the global protocol.

The formula above is provable, thus we know the protocol can terminate successfully.
In the above protocol we know also that all the prepare events happen before the all the commit events. This matches the main requirement of a Two Phase Commit protocol, i.e.\ that all participants successfully prepare a transaction before any participant commits a transaction.
\end{comment}

\subsection{The Additive Operators: Internal and external choice}
\label{section:additives}

The multiplicative operators and the additive operators $\wwith$ and $\ooplus$ %together with $\top$ and $0$
form the sub-system $\textsf{MAV}$~\cite{Horne2015}.

\paragraph{Note on atoms.}
The sub-system \textsf{MAV} has been proposed as a semantics for session types~\cite{Ciobanu2015}, where atoms are the types of messages exchanged preordered by any subtype system.
This presentation of \textsf{MAV}, differs from the session type approach only in that atoms are: either channels that carry terms rather than types, with an equivalence relation over terms; or tests, ordered by classical implication. This is due to the intention to achieve a modelling expressive power comparable to the finite applied $\pi$-calculus. 

Equivalence relations, classical implication and subtyping relations are all preorders. It happens that, for consistency, the only necessary property of atoms is that they are preordered. %(preserved by substitution).
Therefore, considerable creativity is permitted when defining atoms.

\paragraph{Internal and external choice.}
The two additive binary operators ``internal choice'' $\ooplus$ and ``external choice'' $\wwith$ model two forms of choice when statically analysing protocols~\cite{Abramsky1993}. Intuitively, an internal choice is a choice that we can make, as the executor of the protocol or designer of the protocol runtime. In contrast, an external choice, is a choice that we cannot predict at compile time, such as a user input or a potential component failure.
%Rules for the additive operators, in Fig.~\ref{figure:spv}, are similar to those in~\cite{Strassburger2002}. 

For making an internal choice, The \textit{left} and \textit{right} rules for internal choice, select either the left or right branch. In the following example an internal choice is made to receive on channel $a$.
\[
\co{a}(\texttt{pk}(sk))
\cpar
\left(
 a(\texttt{pk}(sk))
 \ooplus
 b(\textit{sk})
\right)
\longrightarrow
\co{a}(\texttt{pk}(sk))
\cpar
a(\texttt{pk}(sk))
\longrightarrow
\cunit
\]
Intuitively, we read $P \wwith Q$ as ``external choice'', where we do not have control over which branch to take.
Because we do not have control we must consider both branch $P$ and branch $Q$ during analysis.
The \textit{distributivity} rule effectively branches two alternative derivations, thereby permitting two separate execution paths to be analysed in parallel. For example, in the following we do not know at compile time whether the message will be sent on channel $a$ or on channel $b$, hence we check both possibilities. 
\[
\begin{array}{l}
\left(
\co{a}(\texttt{pk}(sk))
\wwith
\co{b}(\textit{sk})
\right)
\cpar
\left(
 a(\texttt{pk}(sk))
 \ooplus
 b(\textit{sk})
\right)
\\~~~~~~~~~~~~
\begin{array}{rl}
\longrightarrow
&
\left(
\co{a}(\texttt{pk}(sk))
\cpar
\left(
 a(\texttt{pk}(sk))
 \ooplus
 b(\textit{sk})
\right)
\right)
\wwith
\left(
\co{b}(\textit{sk})
\cpar
\left(
 a(\texttt{pk}(sk))
 \ooplus
 b(\textit{sk})
\right)
\right)
\\
\longrightarrow
&
\left(
\co{a}(\texttt{pk}(sk))
\cpar
 a(\texttt{pk}(sk))
\right)
\wwith
\left(
\co{b}(\textit{sk})
\cpar
\left(
 a(\texttt{pk}(sk))
 \ooplus
 b(\textit{sk})
\right)
\right)
\\
\longrightarrow
&
\left(
\co{a}(\texttt{pk}(sk))
\cpar
 a(\texttt{pk}(sk))
\right)
\wwith
\left(
\co{b}(\textit{sk})
\cpar
 b(\textit{sk})
\right)
\\
\longrightarrow
&
\cunit
\wwith
\left(
\co{b}(\textit{sk})
\cpar
 b(\textit{sk})
\right)
\longrightarrow
\cunit
\wwith
\cunit
\longrightarrow
\cunit
\end{array}
\end{array}
\]
The \textit{tidy branch} rule can only be triggered if both paths can be successfully closed, indicating the possibility of successful execution regardless of the branch selected. 
%This allows us to cover both possible branches of the external choice.

\begin{comment}
\paragraph{The top and bottom predicates.}
The top predicate $\top$ and bottom predicate $0$ are both distinct from $\cunit$. Bottom $0$ intuitively represent deadlock, and is distinguished from $\cunit$, by having neither \textit{close} rules nor playing a special rule in the semantics. Equivalently, it can be seen as the \textit{false} test that can never be satisfied.
%
The $\top$ predicate is the predicate that is free to behave as any predicate. This is useful for static analysis. For example, we can state predicates such as, ``after receiving a secret we don't care what happens'', as follows: $a(\textit{secret}) \cseq \top$.
% Possibly save until implication is introduced.
For example, the following derivation holds.
\[
\begin{array}{rl}
\left(a(\textit{secret}) \cseq \top\right)
\cpar
\left(\co{a}(\textit{secret}) \cseq b(\textit{OK})\right)

\longrightarrow & \left(a(\textit{secret}) \cpar \co{a}(\textit{secret}) \right) \cseq
\left(\top \cpar b(\textit{OK})\right) \\
\longrightarrow & \left(\top \cpar b(\textit{OK})\right) 
\longrightarrow \top \longrightarrow \cunit 
\end{array}
\]
In the above derivation, once the predicate on the left of the parallel composition receives the secret from the other process, it doesn't matter what happens. Effectively, the acknowledgement on channel $b$ is ignored, but without affecting the successful execution of the protocol.
\end{comment}

\paragraph{Example of a protocol with choice.}
Consider a protocol that is part of a write transaction on a distributed file system~\cite{Ghemawat2003}.
In this protocol, three nodes must finalise a write such that the data is consistent. If there is a failure at one replica, then the write is retried once more.
A predicate representing part of the protocol is presented below.
\[
\begin{array}{rl}
&
\co{\textit{write}}
\cseq
\left(
\textit{error} \ooplus \textit{complete}
\right)
\\
\cpar
&
\textit{write}
\cseq
\left(
 \co{\textit{try}} \cpar 
 \co{\textit{try}}
\right)
\cseq
\left(
 \begin{array}{l}
 \left(
  \left(
   \textit{OK} \tensor \textit{OK}
  \right)
  \cseq
  \co{\textit{complete}}
 \right)
 \ooplus \\
 \left(
  \begin{array}{l}
  \left(
   \textit{KO} \tensor \top
  \right)
  \cseq 
  \left(
   \co{\textit{try}} \cpar 
   \co{\textit{try}}
  \right)
  \cseq \\
  \left(
  \begin{array}{l}
  \left(
   \left(
    \textit{OK} \tensor \textit{OK}
   \right)
   \cseq
   \co{\textit{complete}}
  \right)
  \ooplus \\
  \left(
   \left(
    \textit{KO} \tensor \top
   \right)
   \cseq
   \co{\textit{error}}
  \right)
  \end{array}
  \right)
\end{array}
 \right)
 \end{array}
\right)
\\
\cpar
&
\textit{try}
\cseq
\left(
 \left(
  \co{\textit{OK}} \cseq
  \left(
   \left(
   \textit{try} \cseq
   \co{\textit{OK}}
   \right)
   \ooplus \cunit
  \right)
 \right)
 \wwith
\left(
 \co{\textit{KO}} \cseq
 \textit{try}
 \cseq
 \left(
  \co{\textit{OK}} \wwith \co{\textit{KO}}
 \right)
\right)
\right)\\
\cpar
&
\textit{try}
\cseq
\left(
 \left(
  \co{\textit{OK}} \cseq
  \left(
   \left(
   \textit{try} \cseq
   \co{\textit{OK}}
   \right)
   \ooplus \cunit
  \right)
 \right)
 \wwith
\left(
 \co{\textit{KO}} \cseq
 \textit{try}
 \cseq
 \left(
  \co{\textit{OK}} \wwith \co{\textit{KO}}
 \right)
\right)
\right)
\end{array}
\]
The above predicate represents four participants in a protocol, described below.
\begin{itemize}
\item The first line represent a client that sends on the \textit{write} channel and receives on either the \textit{complete} or \textit{error} channel. Note that, for simplicity, values on channels are omitted in this example. The messages communicated can be made explicit by using quantifiers in the next section.

\item The second line represents a primary replica. The primary replica receives on the \textit{write} channel, then sends on the \textit{try} channel of two secondary replicas. Either both replicas respond on the \textit{OK} channel, represented by $\textit{OK} \tensor \textit{OK}$, or at least one responds with $\textit{KO}$, represented by $\textit{KO} \tensor \top$. If both replicas respond on the \textit{OK} channel, then the client is notified on the \textit{complete} channel. Otherwise, there may be an inconsistency, hence the two replicas are both retried. If, after retrying, there is still a \textit{KO} message, then the \textit{error} channel is used to notify the client.

\item The last two lines of the predicate above represent the secondary replicas. These replicas wait on the \textit{try} channel, then either respond on the \textit{KO} or \textit{OK} channel. Notice that an external choice is used at this point, indicating that we do not know at compile time which branch will be selected. Even if \textit{OK} is sent, the operation may be retried, hence there is the option to respond to another \textit{try} request. The fact that the retry is optional is indicated by the internal choice that allows the selection of the unit when no retry arrives.
\end{itemize}

There is a derivation from the above predicate to $\cunit$. An intermediate step is presented below, where the first external choices have been distributed amongst each other.
\[
\begin{array}{rl}
&
\textit{error} \ooplus \textit{complete}
\\
\cpar
&
\left(
 \begin{array}{l}
 \left(
  \left(
   \textit{OK} \tensor \textit{OK}
  \right)
  \cseq
  \co{\textit{complete}}
 \right)
 \ooplus \\
 \left(
  \left(
   \textit{KO} \tensor \top
  \right)
  \cseq
  \left(
   \co{\textit{try}} \cpar 
   \co{\textit{try}}
  \right)
  \cseq
  \left(
  \begin{array}{l}
  \left(
   \left(
    \textit{OK} \tensor \textit{OK}
   \right)
   \cseq
   \co{\textit{complete}}
  \right)
  \ooplus \\
  \left(
   \left(
    \textit{KO} \tensor \top
   \right)
   \cseq
   \co{\textit{error}}
  \right)
  \end{array}
  \right)
 \right)
 \end{array}
\right)
\\
\cpar
&
\left(
\begin{array}{rl}
\left(
 \left(
  \co{\textit{OK}} \cseq
  \left(
   \left(
    \textit{try} \cseq
    \co{\textit{OK}}
   \right)
   \ooplus \cunit
  \right)
 \right)
 \cpar
 \left(
  \co{\textit{OK}} \cseq
  \left(
   \left(
    \textit{try} \cseq
    \co{\textit{OK}}
   \right)
   \ooplus \cunit
  \right)
 \right)
\right)
&
\wwith
\\
\left(
 \left(
  \co{\textit{OK}} \cseq
  \left(
   \left(
    \textit{try} \cseq
    \co{\textit{OK}}
   \right)
   \ooplus \cunit
  \right)
 \right)
 \cpar
\left(
 \co{\textit{KO}} \cseq
 \textit{try}
 \cseq
 \left(
  \co{\textit{OK}} \wwith \co{\textit{KO}}
 \right)
\right)
\right)
&
\wwith
\\
\left(
\left(
\left(
 \co{\textit{KO}} \cseq
 \textit{try}
 \cseq
 \left(
  \co{\textit{OK}} \wwith \co{\textit{KO}}
 \right)
\right)
\cpar
\left(
 \co{\textit{KO}} \cseq
 \textit{try}
 \cseq
 \left(
  \co{\textit{OK}} \wwith \co{\textit{KO}}
 \right)
\right)
\right)
\right)
\end{array}
\right)
\end{array}
\]
A subsequent state in the derivation is the following.
\[
\begin{array}{rl}
&
\textit{error} \ooplus \textit{complete}
\\
\cpar
&
\left(
\begin{array}{rl}
&
\co{\textit{complete}}
\\
\wwith
&
\left(
 \begin{array}{rl}&
 \left(
   \begin{array}{l}
   \left(
    \left(
     \textit{OK} \tensor \textit{OK}
    \right)
    \cseq
    \co{\textit{complete}}
   \right)
   \ooplus \\
   \left(
    \left(
     \textit{KO} \tensor \top
    \right)
    \cseq
    \co{\textit{error}}
   \right)
   \end{array}
 \right)
 \\
 \cpar&
 \left(
  \left(
   \co{\textit{OK}} \cpar \co{\textit{OK}}
  \right)
  \wwith
  \left(
   \co{\textit{OK}} \cpar \co{\textit{KO}}
  \right)
 \right)
 \end{array}
\right)
\\
\wwith
&
\left(
 \begin{array}{rl}
 &
 \left(
   \begin{array}{l}
   \left(
    \left(
     \textit{OK} \tensor \textit{OK}
    \right)
    \cseq
    \co{\textit{complete}}
   \right)
   \ooplus \\
   \left(
    \left(
     \textit{KO} \tensor \top
    \right)
    \cseq
    \co{\textit{error}}
   \right)
   \end{array}
 \right)
 \\
 \cpar&
 \left(
  \left(
   \co{\textit{OK}} \cpar \co{\textit{OK}}
  \right)
  \wwith
  \left(
   \co{\textit{OK}} \cpar \co{\textit{KO}}
  \right)
  \wwith
  \left(
   \co{\textit{KO}} \cpar \co{\textit{KO}}
  \right)
 \right)
 \end{array}
\right)
\end{array}
\right)
\end{array}
\]
Notice that there are six independent branches to explore (two being identical). In this example, all branches have a derivation ending with the unit, hence the whole protocol may complete regardless of the branches selected. In general, the worst case is that there are exponentially many branches compared to the size of the predicate.



\begin{comment}

The protocol prepares with a some value and commits with a function applied to that value.
To demonstrate choice, the protocol may abort before completing the prepare stage. The effect is that the transaction may be rolled back. The following is provable, hence the protocol terminates regardless of whether the transaction commits or aborts.
%
\[
\begin{array}{c}
%\left(
 %\textit{begin} \cseq
 \left(
    \cforall{u} \co{\textit{prepare}(u)} \ooplus \textit{abort}
 \right)
%\right)
\cpar
\\
%\textit{begin}
\left(
  \cexists{x} \left(
     \textit{prepare}(x) \cseq \co{\textit{commit}(latest(x))}
  \right)
  \wwith
  \left(
   \co{\textit{abort}}
   \tensor
   \co{\textit{abort}}
  \right)
\right)
\cpar
\\
%\left(
% \co{\textit{begin}} \cseq
 \left(
    \cexists{y} \textit{commit}(y)
    \ooplus
    \textit{abort}
 \right)
%\right)
\end{array}
\]
%
Consider the above protocol line by line in more detail. There are three roles, a participant, leader and client.
\begin{itemize}
\item The first line represents a participant where there are two possibilities. The first possibility is an observable \textit{prepare} event with an external term $u$. The other possibility is that the participant observes an \textit{abort} event. The choice is internal, since the choice can be determined in reaction to the behaviour of the leader. 
\item The second line represents a leader which drives the transaction. One possibility is that the transaction observes the \textit{prepare} event before a \textit{commit}. A function of the term observed in the \textit{prepare} event is observable in the \textit{commit} event. 
The other possibility is that leader chooses to gives up waiting for the participant and triggers \textit{abort} events.
The choice is external, since we cannot determine at compile time what the leader with chose to do.
\item The third line represent the client. The client chooses to commits or abort based on the behaviour of the leader.
\end{itemize}

As in the previous example, we can determine what values are communicated. If the client observes the \textit{commit} event, then we know the term observed is a function of the external term transmitted by the participant. Effectively, $x$ is unified with $latest(u)$ when a substitution is applied, for any value of $u$. If the client observes the \textit{abort} event, no term is communicated.
\end{comment}




%The additives and first-order quantifiers are introduced in the following paragraphs. 
%Firstly, we introduce the first order quantifiers `exists' and `forall'. Secondly, we introduce the additive binary connectives `with' and `plus'. 
%In Section~\ref{section:multiplicatives} we introduce the multiplicative binary operators `tensor', `par' and `seq'.
%We refer to formulae in the calculus as processes due to their intuitive interpretation as truly concurrent processes.


\begin{comment}
\begin{gather*}
\vlinf{}{}{
 x = x
}{
 \cunit
}
\qquad
\vlinf{}{}{
 \nfv{x}{(P \vlodot Q)}
}{
 \nfv{x}{P} \tensor  \nfv{x}{Q}
}
\qquad
\vlinf{}{}{
 \nfv{x}{\quantifier{y}P}
}{
 (x = y) \ooplus (\nfv{x}{P})
}
\end{gather*}
\end{comment}





%A deductive system defines rewrites over formulae. We assume that a deductive rule can be applied in any context. It may be helpful to read deductive rules upwards, where the conclusion below the line is rewritten to the premise above the line. If the topmost premise is the unit, then we have a proof of the conclusion.

\begin{comment}
%\begin{figure}[h]
\begin{gather*}
\vlinf{\ainteractdown}{}{
 \context{
  \co{A} \cpar A
 }
}{
 \context{
  \cunit
 }
}
\qquad\qquad
\vlinf{\seqdown}{}{
\context{
 \left(P \cthen R\right)
 \cpar
 \left(Q \cthen S\right)
}
}{
\context{
 \left(P \cpar Q\right)
 \cthen
 \left(R \cpar S\right)
}
}
\qquad\qquad
\vlinf{\switch}{}{
\context{
 P \cpar \left(Q \tensor R\right)
}
}{
\context{
 \left(P \cpar Q\right) \tensor R
}
}
\\[12pt]
\vlinf{\ainteractup}{}{
\context{
 \cunit
}
}{
\context{
 \co{A} \tensor A
}
}
\qquad\qquad\qquad
\vlinf{\sequp}{}{
\context{
 \left(P \tensor Q\right)
 \cthen
 \left(R \tensor S\right)
}
}{
\context{
 \left(P \cthen R\right)
 \tensor
 \left(Q \cthen S\right)
}
}
\end{gather*}
%\caption{Rewrite rules for the multiplicative binary operators: $P$,$Q$ and $R$ are processes and $A$ is an atom.}
%\label{figure:multiplicatives}
%\end{figure}
\end{comment}

%A positive atom and a negative atom can interact over a ``par'' resulting in the unit. This is expressed by the \textit{atomic interact} rule $\inlinerule\ainteractdown$. Such interactions are similar to interaction in Milner's CCS~\cite{Milner1982}, where an atom and complementary atom can interact resulting in a silent action. The connection between CCS and \textsf{BV} has been explored by Bruscoli~\cite{Bruscoli2002}.

%The fragment consisting of ``par'' and ``tensor'' is multiplicative linear logic (with mix). The multiplicative operators control interaction in complementary ways. The ``par'' operator represents parallel composition were atoms on the left may interact with atoms on the right. In contrast the tensor product means that nothing on the left can interact with anything on the right. The \textit{switch} rule $\inlinerule\switch$ refines where interaction may take place. In the conclusion of the rule noting in $R$ may interact with anything in $Q$, but in the premise nothing in $R$ may interact with anything in $P$ or $Q$.

%Pomsets are the classic true concurrency model. Unlike interleaving models of concurrency, pomsets do not enforce unnecessary dependencies on the order in which parallel actions occur. 

%For every rule in \textsf{BV} there is a complementary rule called a corule. The rules with the corules $\inlinerule\ainteractup$ and $\inlinerule\sequp$ form the system Symmetric \textsf{BV} (\textsf{SVB}). A theorem by Guglielmi~\cite{Guglielmi2007} proves that the corules are admissible, which fulfils the role of a cut elimination theorem that establishes the internal consistency of the proof system \textsf{BV}.
%
\begin{comment}
!! only include if used !!
\begin{theorem}[Cut elimination~\cite{Guglielmi2007}]
\label{theorem:Guglielmi}
The cointeract and cosequence rules are admissible, for provable processes in the system SBV.
\end{theorem}
\end{comment}

%Note that a motivation for using a framework based on linear logic rather than classical logic for modelling updates is similar to the motivation for linear constraint programs~\cite{Best1997}. In classical constraint programs (in this case constraints are data tuples) we can always add more constraints, until we add an inconsistent constraint at which point everything is trivially true. However, since linear logic is resource sensitive, we can also remove constraints. Girard argues that the classical non-monotonic approach to updates, where belief is revised to avoid inconsistencies, has had limited success~\cite{Girard1995}.


\subsection{The First-order Quantifiers: Receiving known and unknown data.}
\label{section:quantifiers}

To obtain the calculus \textsf{MAV1}, the calculus \textsf{MAV} is extended with first-order quantifier~\cite{Brunnler2006} that range over all terms, as expected. A simple type system can be devised to ensure variables are properly used in tests.

\paragraph{A novel intuition.}
We provide a novel intuition for first-order quantifiers, that complements the external/internal choice intuition for the additives. Quantifiers represent a choice of substitutions of variables for terms. Existential quantification represent an internal choice in the sense that we, as executors of the protocol, have control over what substitution we choose.
In contrast, for universal quantification the intuition is that at compile time we do not know what substitution will be chosen (due to a user input or the random generation of a nonce for example); hence for static analysis we must investigate all possible substitutions.
%
The rule \textit{select} can be applied to make the internal choice of substitution. For example, consider the following derivation that models the input of the term $\texttt{senc}(k,m)$ on channel $b$.
\[
\begin{array}{l}
\co{a}(\texttt{senc}(k,m))
\cpar
\exists x \left(a(x) \cseq P\right) \\
\qquad
\begin{array}{rl}
\longrightarrow &
\co{a}(\texttt{senc}(k,m))
\cpar
\left(a(\texttt{senc}(k,m)) \cseq P\sub{x}{\texttt{senc}(k,m)}\right)
\\
\longrightarrow &
\left(
\co{a}(\texttt{senc}(k,m))
\cpar
a(\texttt{senc}(k,m)) \right) \cseq P\sub{x}{\texttt{senc}(k,m)}
\\
\longrightarrow &
P\sub{x}{\texttt{senc}(k,m)}
\end{array}
\end{array}
\]
Observe above that the exists quantifier serves a similar role to the input binder in the applied $\pi$-calculus. The effect is that the term $\texttt{senc(k,m)}$ is passed to the continuation predicate~$P$.

The rule \textit{extrude} expands the scope of a universal quantifier as long as the name is free. Notice the similarity to expanding a scope using a structural congruence in name passing process calculi. Indeed we can model the effect of passing an ``external'' name, by combining the select and extrude rules as follows, assuming that $\nfv{y}{P}$.
\[
\begin{array}{l}
\forall y \left(
\co{a}(\texttt{senc}(y,m))
\right)
\cpar
\exists x \left(a(x) \cseq P\right)
\\\qquad
\begin{array}[t]{rl}
\longrightarrow &
\forall y \left(
\co{a}(\texttt{senc}(y,m))
\cpar
\exists x \left(a(x) \cseq P\right)
\right)
\\
\longrightarrow &
\forall y \left(
\co{a}(\texttt{senc}(y,m))
\cpar
\left(a(\texttt{senc}(y,m)) \cseq P\sub{x}{\texttt{senc}(y,m)}\right)
\right)
\\
\longrightarrow &
\forall y \left(
\left(
\co{a}(\texttt{senc}(y,m))
\cpar
a(\texttt{senc}(y,m))
\right)
\cseq P\sub{x}{\texttt{senc}(y,m)}
\right)
\\
\longrightarrow &
\forall y \left(
P\sub{x}{\texttt{senc}(y,m)}
\right)
\end{array}
\end{array}
\]
Notice that the effect is that, as in the previous example, the term $\texttt{senc}(y,m)$ is communicated to the process $P$. The extrude rule expanding the scope of the universal quantifier enables the term $y$, unknown at compile time, to be communicated.

The \textit{close scope} rule intuitively mean that, if a protocol inside a universal quantifier can successfully close without instantiating the bound variable, then the protocol can close for all possible substitutions.
For example, consider the following protocol.
\[
\forall x \left(
 \co{a}(pk(x)) \cseq \co{b}(\texttt{aenc}(x,m))
\right)
 \cpar
\exists y \left(
 a(y) \cpar 
 \exists z \left(
  b(z) \cpar (\texttt{adec}(y,z) = m)
 \right)
\right)
\]
By assuming the following equation as part of the equational theory over the signature of functions, there exists a derivation ending with $\cunit$, representing successful termination.
\[
\texttt{adec}(\texttt{pk}(x), \texttt{aenc}(x,y)) = y
\]
The above equation, from work on applied $\pi$-calculus, models the decryption of a message $y$ that was encoded using secret key $x$, by using corresponding public key $\texttt{pk}(x)$.

As demonstrated above, universal quantification can partially fulfil the role of the new name quantifiers in the applied $\pi$-calculus. However none of the quantifiers in this calculus is an exact match for new name.
%since there is always a predicate that can discover the bound variable, when composed in paralel.
%We argue that this is acceptable, since security properties are investigated we are forced to employ cryptographic primitives to reason about 

\begin{comment}
\textit{Renaming operator.}
%there are occassions where a nominal quantifier is more appropriate.
We introduce a nominal quantifier provisionally named \textit{rename} with the symbol $\rename{}$ (the symbol also acknowledges that Roversi~\cite{Roversi2011} introduced the operator). The renaming operator, models an opaque name that is public. Hence the variable bound by a renaming quantifier can be swapped with any name that does not appear as a constant. Consider the following two predicates.
\[
\exists y. \rename{x} .\left(
 a\;f(x,y) \tensor b\;g(x,y)
\right)
\cpar
\rename{x}.\left(
 \co{a}\;f(x,d)
 \cpar
 \co{b}\;g(x,d)
\right)
\]
\[
\exists y. \rename{x} .\left(
 a\;x \tensor b\;f(c,x)
\right)
\cpar
%\left(
 \co{a}\;f(c,d)
 \cpar
 \co{b}\;g(c,d)
%\right)
\]
The first predicate has a derivation to $\cunit$, but the second does not. Thus the two synchronised inputs on the left will only accept a renameable term for $x$. Notice also the scope of the existential quantifier indicating that the bound variable must be instantiated with the same variable in both inputs. In \cite{Horne2014} this technique enables rich queries to be expressed.



The nominal quantifier $\rename{}$ is closest to the new quantifier $\new$~\cite{Pitts03}, since it is also self-dual and strictly stronger than existential quantification, but strictly weaker than universal quantification. The quantifier does not match the nominal quantifier $\nabla$~\cite{Tiu2009}, since $\nabla$ is not between existential and universal quantification.
\end{comment}

\paragraph{Example of commit protocol.}
Consider a commit protocol, inspired by part of Google Spanner's write protocol~\cite{Corbett2012}. This instance, with one leader and two participants, uses three values that are not known in advance (indicated by bound variables $u$, $v$ and $w$), and then commits the max of these values plus $1$.
%
\[
\begin{array}{rl}
&\forall{u}. \left(\co{\textit{prepare}}(u)\right)
\cseq \exists z. \left(\textit{commit}(z) \tensor (u < z) \right)
\\
\cpar
&
\forall{v}. \left(\co{\textit{prepare}}(v)\right)
\cseq \exists z. \left(\textit{commit}(z) \tensor (v < z) \right)
\\
\cpar
&
\exists{x}. \exists{y}.
\forall{w}.
\left(
 \begin{array}{l}
 \left(\textit{prepare}(x) \tensor \textit{prepare}(y)\right) \cseq
 \\
 \left(
 \begin{array}{rl}
       &\co{\textit{commit}}(\texttt{max}(x,y,w) + 1) \\
 \cpar &\co{\textit{commit}}(\texttt{max}(x,y,w) + 1)
 \end{array}
 \right)
 \end{array}
\right)
%\\ \cpar & \exists{z}. \textit{commit}(z)
\end{array}
\]
Assume that, in tests, we have inequality predicates and the expected equational theory for \texttt{max} and addition over the natural numbers. 
If we consider the substitutions we can statically determine the values that are transmitted at various points in the protocol. Consider the above example line-by-line.
\begin{itemize}
\item The first two lines represents two participants that output a term on channel \textit{prepare}. The output term is not known at compile-time, hence are universally bound variables $u$ and $v$.
The participants are then ready to input a term on channel \textit{commit}. The test checks that the input term is strictly greater than the term output on the \textit{prepare} channel.

\item The rest of the predicate represent a leader that synchronously inputs two messages on channel \textit{prepare}, then sends two messages on channel \textit{commit}.
The term output on both commit channels is one greater than the maximum of the two values input, and a third value unknown at compile time, represented by $w$.
%\item The third line represents a client that observes the \textit{commit} event. The variable $z$ is unified with the term $\texttt{max}(u,v)$. The intuition is that, when the protocol commits, the client observes max applied the terms which are chosen for $u$ and $v$ at runtime.
\end{itemize}

\noindent Due to the use of universal quantification, we are able to evaluate the termination of the protocol without knowing some of the values transmitted, and perform tests comparing values sent and received.
%This style of modelling is similar in spirit to the use of session types, which can also be given a logical foundation where termination can be evaluated statically~\cite{Caires2010}. 
%Future work includes to using \textsf{PV} as a foundation for behavioural type systems.




\begin{comment}
\begin{gather*}
\vlinf{\instantiatedown}{}{
\context{
 \cexists{x} P
}
}{
\context{
 P\sub{x}{v}
}
}
\qquad\qquad\quad
\vlinf{\freedown}{\nfv{x}{R}}{
\context{
 R
}
}{
\context{
 \cexists{x} R
}
}
\qquad\qquad\quad
\vlinf{\retractdown}{}{
\context{
 \cforall{x} P \cpar \cexists{x} Q
}
}{
\context{
 \cforall{x} (P \cpar Q)
}
}
\\[12pt]
\vlinf{\instantiateup}{}{
\context{
 P\sub{x}{v}
}
}{
\context{
 \cforall{x} P
}
}
\qquad\qquad\quad
\vlinf{\freeup}{\nfv{x}{R}}{
\context{
 \cforall{x} R
}
}{
\context{
 R
}
}
\qquad\qquad\quad
\vlinf{\retractup}{}{
\context{
 \cexists{x} (P \tensor Q)
}
}{
\context{
 \cexists{x} P \tensor \cforall{x} Q
}
}
\end{gather*}
\end{comment}



\begin{comment}
\subsection{Examples}



Combining the above techniques we can model a full two phase commit protocol, where the participants are:

1. The client that initiates the transaction by contacting the leader and participants with their workload. At the end the client receives the commit or abort message.

2. The lead server that receives prepare time stamps from participant servers. Once it received prepare timestamps from everyone, it waits until the timestamp has passed, then sends commit messages to the client and participants. The leader drives aborts.

3. The participants, that notify the leader with a prepare timestamp and receives a commit message.

\end{comment}


